High-Accuracy and Efficient DV-Hop Localization for IoT Using Hop Loss

Accurate localization is critical for Internet of Things (IoT) applications. Using hop loss in DV-Hop-based algorithms is a promising approach. Nevertheless, challenges lie in overcoming the computational complexity caused by re-calculating the predicted hop-counts, and how to further optimize the modeling for better accuracy. In this paper, a novel hop loss modeling, distance-based connectivity consistency (DCC), is proposed. By focusing on the first order connectivity, DCC avoids computing predicted hop-counts, and significantly reduces the time complexity. We also provide a proof to theoretically guarantee that this design achieves a full coverage of all hop errors. In addition, by computing a continuous loss function instead of the discrete hop-count errors, DCC further improves the localization accuracy. In the evaluations, DCC demonstrates notable improvements in accuracy over other highly regarded algorithms, and reduces 30% to 40% total computation time compared with the baseline algorithm using hop loss.

==> images/ac_base_fail_case/pred.tex <==
\begin{tikzpicture}
        \def\normalsize{0.5pt}
        \def\hightlightsize{2pt}
        \def\length{2.5}
        \def\width{0.5}
        \def\height{1.5}
        \def\radius{1.5}
        \definecolor{magenta}{RGB}{255,0,255}
        % Loop through to generate random coordinates and draw dots

        \coordinate (dot1) at (0, 0);
        \coordinate (dot2) at ($(dot1) + (0.7 * \radius, 0.2 * \radius)$);
        \coordinate (dot3) at ($(dot2) + (0.65 * \radius, -0.25 * \radius)$);
        \coordinate (dot4) at ($(dot3) + (0.7 * \radius, +0.2 * \radius)$);
        \coordinate (titleReal) at ($(dot1) + (1.0 * \radius, 1.2 * \radius)$);

        % \draw(dot1) -- (dot2);
        % \draw(dot2) -- (dot3);
        % \draw(dot3) -- (dot4);
       
        % \node at (titleReal) {Real};
        % \filldraw[blue] (dot1) circle (\hightlightsize) node[above left, text=black] {1};
        % \filldraw[blue] (dot2) circle (\hightlightsize) node[below, text=black] {2};
        % \filldraw[blue] (dot3) circle (\hightlightsize) node[above, text=black] {3};
        % \filldraw[blue] (dot4) circle (\hightlightsize) node[below, text=black] {4};


         \coordinate (dot5) at ($(dot4) + (1.5 * \radius, -0.5 * \radius)$);
        \coordinate (dot6) at ($(dot5) + (0.9 * \radius, -0.05 * \radius)$);
        \coordinate (dot7) at ($(dot6) + (-0.05 * \radius, 0.9 * \radius)$);
        \coordinate (dot8) at ($(dot7) + (-0.9 * \radius, 0.05 * \radius)$);
        \coordinate (titlePred) at ($(titleReal) + (3 * \radius, 0)$);
        %\coordinate (dotend) at (-0.8*\length, -\width * 0.5 - \height * 2);

        \draw(dot5) -- (dot6);
        \draw(dot6) -- (dot7);
        \draw(dot7) -- (dot8);
        \draw(dot8) -- (dot5);
       
        %\node at (titlePred) {Prediction};
        \filldraw[blue] (dot5) circle (\hightlightsize) node[below left, text=black] {1};
        \filldraw[blue] (dot6) circle (\hightlightsize) node[below, text=black] {2};
        \filldraw[blue] (dot7) circle (\hightlightsize) node[right, text=black] {3};
        \filldraw[blue] (dot8) circle (\hightlightsize) node[left, text=black] {4};
        
    \end{tikzpicture}

==> images/ac_base_fail_case/real.tex <==
\begin{tikzpicture}
        \def\normalsize{0.5pt}
        \def\hightlightsize{2pt}
        \def\length{2.5}
        \def\width{0.5}
        \def\height{1.5}
        \def\radius{1.5}
        \definecolor{magenta}{RGB}{255,0,255}
        % Loop through to generate random coordinates and draw dots

        \coordinate (dot1) at (0, 0);
        \coordinate (dot2) at ($(dot1) + (0.7 * \radius, 0.2 * \radius)$);
        \coordinate (dot3) at ($(dot2) + (0.65 * \radius, -0.25 * \radius)$);
        \coordinate (dot4) at ($(dot3) + (0.7 * \radius, +0.2 * \radius)$);
        \coordinate (titleReal) at ($(dot1) + (1.0 * \radius, 1.2 * \radius)$);

        \draw(dot1) -- (dot2);
        \draw(dot2) -- (dot3);
        \draw(dot3) -- (dot4);
       
        %\node at (titleReal) {Real};
        \filldraw[blue] (dot1) circle (\hightlightsize) node[above left, text=black] {1};
        \filldraw[blue] (dot2) circle (\hightlightsize) node[below, text=black] {2};
        \filldraw[blue] (dot3) circle (\hightlightsize) node[above, text=black] {3};
        \filldraw[blue] (dot4) circle (\hightlightsize) node[below, text=black] {4};
        
    \end{tikzpicture}
